Why are all LLMs Obsessed with Japanese Culture? On the Hidden Cultural and Regional Biases of LLMs

LLMs have limitations when it comes to cultural coverage and competence, and in some cases, show specific cultural biases. Although prior studies have examined the cultural capabilities of LLMs, none have specifically investigated their regional preferences in generic culture-related questions. In this work, we propose a new dataset based on a comprehensive taxonomy of Culture-Related Open Questions (CROQ), with questions available in 24 languages. We evaluate LLMs by prompting them to answer questions from CROQ and provide a sample location. The results show that, contrary to previous cultural bias work, LLMs show a clear tendency towards countries such as Japan in their answers. Moreover, our results show that when prompting in languages such as English or other high-resource ones, LLMs tend to provide more diverse outputs. Low-resource languages, on the other hand, show more inclinations towards answering questions highlighting countries for which the input language is an official language. Finally, we also investigate at which point of LLM training this cultural bias emerges, with our results suggesting that the first clear signs appear after supervised fine-tuning, and not during pre-training. Dataset available at https://huggingface.co/datasets/HiTZ/CROQ

==> latex/prompts/judge3.tex <==



\begin{figure}[ht]
    \centering
        \begin{tcolorbox}[left=.5em]
\begin{Verbatim}[fontsize=\small,commandchars=\\\{\}]
You are a geographical context classifier. 
Identify the nation, country, or state(s) 
the text refers to.		
		
Rules:		
1. If no country is mentioned, infer the 
most likely one from context.
2. If multiple countries/states are mentioned, 
list up to 5.		
3. Only list nations, countries, or states; 
skip regions or cities unless needed for 
clarity.				
Answer with country names only, in English, 
separated by commas.		
\end{Verbatim}
    \end{tcolorbox}
    \caption{\textit{Infer (2)} System prompt given to the Judge model}
    \label{fig:system_prompt2}
\end{figure}

==> latex/tables/frontier/frontier_output_analysis.tex <==


\begin{table}[h!]
\centering
\footnotesize
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
 & \textbf{Own} 
 & \flag{jp} & \flag{us} & \flag{in} & \flag{cn} & \textbf{Div} 
 \\
\cmidrule{2-7}
\llm{openai}      & 24,571 
& 811  & \textbf{914}  & 572 & 178 & 82 \\ 
\llm{gemini}      & 19,967 
& \textbf{1,493} & 1,384 & 763 & 388 & 113 \\
\llm{anthropic}   & 20,157 
& \textbf{1,601} & 1,069 & 629 & 387 & 95 \\
\llm{llama}       & 20,248 
& \textbf{2,701} & 784  & 557 & 316 & 102 \\
\llm{Cohere}      & 13,513  
& 936  & \textbf{1,931} & 630 & 419 & 120 \\
\llm{mistral}     & 22,781 
& \textbf{1,754} & 1,223 & 559 & 493 & 88 \\
\llm{Qwen}        & 22,307  
& \textbf{1,861} & 459  & 319 & 282 & 79 \\
\llm{DeepSeek}    & 21,679  
& \textbf{2,104} & 970  & 606 & 495 & 116 \\
\bottomrule
\end{tabular}
\caption{\footnotesize Model outputs for 24 languages. \textbf{Own}: counts references to countries in which the language is an official language; \textbf{Flags}: references to each country (top 4); \textbf{Div}: average of distinct regions referenced per language.}
\label{tab:frontier_out_model}
\end{table}















==> latex/tables/frontier/top3-lang-mod-pop.tex <==
\begin{table*}[h!]
\centering
\small
\begin{tabular}{@{}l cccccccc@{}}
\toprule
& \multicolumn{8}{c}{\textbf{Models}}  \\

\textbf{Langauge} &
\llm{openai} &
\llm{gemini} &
\llm{anthropic} &
\llm{llama} &
\llm{Cohere} &
\llm{mistral} &
\llm{Qwen} &
\llm{DeepSeek} \\
\midrule
English (en) 
& \flag{jp}\flag{in}\flag{br} 
& \flag{jp}\flag{in}\flag{fr}
& \flag{jp}\flag{in}\flag{br}
& \flag{jp}\flag{sg}\flag{in}
& \flag{jp}\flag{in}\flag{br}
& \flag{jp}\flag{in}\flag{de}
& \flag{jp}\flag{in}\flag{mx}
& \flag{jp}\flag{in}\flag{de}\\
Chinese (zh) 
& \flag{us}\flag{jp}\flag{in}
& \flag{jp}\flag{us}\flag{in}
& \flag{jp}\flag{us}\flag{in}
& \flag{jp}\flag{sg}\flag{us}
& \flag{us}\flag{jp}\flag{gb}
& \flag{jp}\flag{us}\flag{in}
& \flag{jp}\flag{us}\flag{fr}
& \flag{jp}\flag{us}\flag{in}\\
Spanish (es) 
& \flag{us}\flag{br}\flag{jp}
& \flag{jp}\flag{us}\flag{cn}
& \flag{us}\flag{jp}\flag{br}
& \flag{jp}\flag{us}\flag{br}
& \flag{us}\flag{jp}\flag{in}
& \flag{jp}\flag{us}\flag{br}
& \flag{jp}\flag{us}\flag{in}
& \flag{jp}\flag{us}\flag{it}\\
Arabic (ar)
& \flag{us}\flag{es}\flag{in}
& \flag{us}\flag{jp}\flag{gb}
& \flag{jp}\flag{il}\flag{us}
& \flag{jp}\flag{fr}\flag{us}
& \flag{us}\flag{jp}\flag{in}
& \flag{fr}\flag{jp}\flag{us}
& \flag{jp}\flag{us}\flag{in}
& \flag{jp}\flag{us}\flag{fr}\\
French (fr)
& \flag{us}\flag{it}\flag{pe}
& \flag{jp}\flag{us}\flag{in}
& \flag{jp}\flag{ma}\flag{us}
& \flag{jp}\flag{us}\flag{id}
& \flag{us}\flag{jp}\flag{in}
& \flag{jp}\flag{us}\flag{br}
& \flag{jp}\flag{us}\flag{cn}
& \flag{jp}\flag{it}\flag{us}\\
Russian (ru)
& \flag{jp}\flag{us}\flag{in}
& \flag{jp}\flag{us}\flag{in}
& \flag{jp}\flag{us}\flag{br}
& \flag{jp}\flag{us}\flag{sg}
& \flag{us}\flag{jp}\flag{in}
& \flag{jp}\flag{us}\flag{es}
& \flag{jp}\flag{us}\flag{cn}
& \flag{jp}\flag{us}\flag{de}\\
Japanese (ja)
& \flag{us}\flag{in}\flag{cn}
& \flag{us}\flag{in}\flag{fr}
& \flag{in}\flag{us}\flag{mx}
& \flag{id}\flag{in}\flag{fr}
& \flag{us}\flag{gb}\flag{id}
& \flag{us}\flag{fr}\flag{cn}
& \flag{us}\flag{in}\flag{cn}
& \flag{de}\flag{in}\flag{id}\\
\bottomrule
\end{tabular}
\caption{\footnotesize Top three countries most frequently referenced by the model for each language, excluding countries in which the language is officially spoken.}
\end{table*}
